False Negative Awareness in Indicator-based Caching Systems

Distributed caching systems such as content distribution networks often advertise their content via lightweight approximate indicators (e.g., Bloom filters) to efficiently inform clients where each datum is likely cached. While false-positive indications are necessary and well understood, most existing works assume no false-negative indications. Our work illustrates practical scenarios where false-negatives are unavoidable and ignoring them significantly impacts system performance. Specifically, we focus on false-negatives induced by indicator staleness, which arises whenever the system advertises the indicator only periodically, rather than immediately reporting every change in the cache. Such scenarios naturally occur, e.g., in bandwidth-constraint environments or when latency impedes each client's ability to obtain an updated indicator. Our work introduces novel false-negative aware access policies that continuously estimate the false-negative ratio and sometimes access caches despite negative indications. We present optimal policies for homogeneous settings and provide approximation guarantees for our algorithms in heterogeneous environments. We further perform an extensive simulation study with multiple real system traces. We show that our false-negative aware algorithms incur a significantly lower access cost than existing approaches or match the cost of these approaches while requiring an order of magnitude fewer resources (e.g., caching capacity or bandwidth).

==> Fig/cachesizeplot.tex <==
% USAGE:
% \cachesizeplot{FILENAME}
% assumes a file FILENAME containing:
% policy  4KAlg   4KBM    4KCF    16KAlg  16KBM   16KCF   64KAlg  64KBM   64KCF
% LRU     1.00    1.20    1.30    1.00    1.40    1.50    1.00    1.60    1.60
% W-tLFU  1.50    1.70    1.60    1.30    1.20    1.40    1.10    1.50    1.70
% FRD     1.60    1.50    1.80    1.30    1.50    1.70    1.20    1.50    1.70
% Hyper   1.60    1.80    1.70    1.40    1.60    1.90    1.50    1.70    1.70% NOTE:
% Alg: our algorithm (bar)
% BM: Static Clairvoyant Benchmark
% CF: Cache first policy
% Note: missing values can be replaced by NaN

\newcommand{\markerone}{*}
\newcommand{\markeronesize}{2pt}
\newcommand{\markertwo}{square}
\newcommand{\markertwosize}{3pt}

\newcommand{\cachesizeplot}[2]{
%
\begin{tikzpicture}
\begin{groupplot}[
    group style=
        {
        group size = 3 by 1,
        xlabels at = edge bottom,
        ylabels at = edge left,
        horizontal sep = 0.02\textwidth,
        vertical   sep = 0.06\textwidth,
        group name=plots,
        },
    major x tick style = transparent,
    ymajorgrids = true,
    width=0.5\columnwidth,
    ytick={1,1.5,2,2.5,3,3.5,4},
    yticklabel style={
        text width=0.035\textwidth,
        align=right,
        inner xsep=0pt,
        xshift=-0.014\textwidth
        },
    ylabel = Normalized Service Cost,
    symbolic x coords= {40, 400, 4000},
    xticklabels =      {40, 400, 4000},
    xticklabel style={
        font=\footnotesize,
        align=center,
        rotate=45,
        yshift=0.012\textwidth
        },
    xtick=data,
    ymin = 0.95,
    ymax= 4,
    legend style={
        legend columns=-1,
        at={(-0.645,1.6)},
        anchor=north,
        /tikz/every even column/.append style={column sep=0.3cm},
        },
    ]

% x       4KAlg   4KBM    4KCF    16KAlg  16KBM   16KCF   64KAlg  64KBM   64KCF
% LRU     1.00    1.20    NaN     1.00    1.40    1.50    1.00    1.60    NaN
% W-tLFU  1.50    1.70    1.60    1.30    1.20    1.40    1.10    1.50    1.70
% FRD     1.60    1.50    1.80    1.30    1.50    NaN     1.20    1.50    1.70
% Hyper   1.60    1.80    1.70    1.40    1.60    NaN     1.50    1.70    1.70

\nextgroupplot[title = Wiki] %, ylabel={arg $|$ cost}]
        % \addplot coordinates {(40,1) (400,2) (4000,3)};% 
        \addplot [ybar = 3pt, fill=cyan!50]  table [ybar, x=policy, y=4KAlg]{#2};
        \addplot [ybar = 3pt, fill=cyan!50]  table [ybar, x=policy, y=4KCF]{#2};
        % \addplot [ybar = 4pt, fill=black!50]  table [ybar, x=policy, y=4KAlg]{#2};
% \nextgroupplot[title = Gradle,yticklabels=\empty]
%         \addplot [ybar = 3pt,fill=cyan!50] table [ybar,x=policy,y=16KAlg]{#2};
% \nextgroupplot[title = Scarab,yticklabels=\empty]
%         \addplot [ybar = 3pt, fill=cyan!50, ybar legend, legend image code/.code={%
%               \draw[] (0cm,-0.1cm) rectangle (0.3cm,0.1cm);
%             },
%         ] table [ybar,x=policy,y=64KAlg]{#2};

\legend{legend}


\end{groupplot}
\end{tikzpicture}
} % end of \newcommand{\cachesizeplot}[1]

% \begin{document}

% \scalebox{0.8}{\cachesizeplot{Scarab}{fig_test4.dat}{F1}{fig_test4.dat}{F2}{fig_test4.dat}{P8}{fig_test4.dat}}
% \pagebreak
% \scalebox{0.8}{\cachesizeplot{Scarab}{fig_test4.dat}{F1}{fig_test4.dat}{F2}{fig_test4.dat}{P8}{fig_test4.dat}}

% \end{document}

